Moduli Stabilization and Stability in Type II/F-theory flux compactifications

In this thesis we study String Theory compactifications to four dimensions focusing on the moduli stabilization process and the associated vacua structure in various frameworks, from Type IIA to F-theory, interpreting the results in the context of the Swampland Program. More specifically, we generalize the bilinear formalism of the scalar potential to include the contributions of geometric fluxes, which we use to perform a systematic search of vacua. We also consider the 10d uplift of AdS4 vacua arising from the 4d massive Type IIA effective theory with only RR and NSNS fluxes. Using the language of SU(3)xSU(3) structures and performing an expansion around the smearing approximation in powers of the string coupling, we study the stability of the SUSY solution and its non-SUSY partner. We contrast the results with the Weak Gravity Conjecture and the AdS instability conjecture in toroidal orbifold examples and find that some non-SUSY cases are in tension with the predictions of those conjectures. From the F-theory perspective, we study moduli stabilization in the complex structure sector of elliptically fibered Calabi-Yau 4-folds in the Large Complex Structure limit. Using homological mirror symmetry, we replicate the analysis for the Type IIA case and give a bilinear expression for the scalar potential, allowing for a detailed study of the vacua structure. We find two distinct families of flux configurations compatible with the tadpole constraints that enable full moduli stabilization. We thoroughly examine the most generic one in the Type IIB limit, where the superpotential is also quadratic and polynomial corrections can be considered at all orders. Finally, we show that at this level of approximation supersymmetric SUSY vacua always contain flat directions. We conclude with a summary of the results and some comments about open questions and future lines of research.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
